Contextualize Me -- The Case for Context in Reinforcement Learning

While Reinforcement Learning ( RL) has made great strides towards solving increasingly complicated problems, many algorithms are still brittle to even slight environmental changes. Contextual Reinforcement Learning (cRL) provides a framework to model such changes in a principled manner, thereby enabling flexible, precise and interpretable task specification and generation. Our goal is to show how the framework of cRL contributes to improving zero-shot generalization in RL through meaningful benchmarks and structured reasoning about generalization tasks. We confirm the insight that optimal behavior in cRL requires context information, as in other related areas of partial observability. To empirically validate this in the cRL framework, we provide various context-extended versions of common RL environments. They are part of the first benchmark library, CARL, designed for generalization based on cRL extensions of popular benchmarks, which we propose as a testbed to further study general agents. We show that in the contextual setting, even simple RL environments become challenging - and that naive solutions are not enough to generalize across complex context spaces.

==> latexmkrc <==

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

$bibtex='bibtex -min-crossrefs=20'

==> tables/context_features/context_features_defaults_bounds.tex <==
\begin{table}
\centering
\caption[Context Features: Defaults and bounds for each environment.]{Context Features: Defaults and Bounds}
\label{tab:context_features_defaults_bounds}
\begin{tabular}{lrll}
\toprule
{} &  Default &                                    Bounds &         Type \\
\midrule
initial\_angle\_lower    &    -0.10 &                               (-inf, inf) &        float \\
initial\_angle\_upper    &     0.10 &                               (-inf, inf) &        float \\
initial\_velocity\_lower &    -0.10 &                               (-inf, inf) &        float \\
initial\_velocity\_upper &     0.10 &                               (-inf, inf) &        float \\
link\_com\_1             &     0.50 &                                    (0, 1) &        float \\
link\_com\_2             &     0.50 &                                    (0, 1) &        float \\
link\_length\_1          &     1.00 &                                 (0.1, 10) &        float \\
link\_length\_2          &     1.00 &                                 (0.1, 10) &        float \\
link\_mass\_1            &     1.00 &                                 (0.1, 10) &        float \\
link\_mass\_2            &     1.00 &                                 (0.1, 10) &        float \\
link\_moi               &     1.00 &                                 (0.1, 10) &        float \\
max\_velocity\_1         &    12.57 &  (1.2566370614359172, 125.66370614359172) &        float \\
max\_velocity\_2         &    28.27 &    (2.827433388230814, 282.7433388230814) &        float \\
torque\_noise\_max       &     0.00 &                               (-1.0, 1.0) &        float \\
force\_magnifier        &    10.00 &                                  (1, 100) &          int \\
gravity                &     9.80 &                                (0.1, inf) &        float \\
initial\_state\_lower    &    -0.10 &                               (-inf, inf) &        float \\
initial\_state\_upper    &     0.10 &                               (-inf, inf) &        float \\
masscart               &     1.00 &                                 (0.1, 10) &        float \\
masspole               &     0.10 &                                 (0.01, 1) &        float \\
pole\_length            &     0.50 &                                 (0.05, 5) &        float \\
update\_interval        &     0.02 &                              (0.002, 0.2) &        float \\
force                  &     0.00 &                               (-inf, inf) &        float \\
goal\_position          &     0.50 &                               (-inf, inf) &        float \\
goal\_velocity          &     0.00 &                               (-inf, inf) &        float \\
gravity                &     0.00 &                                  (0, inf) &        float \\
max\_position           &     0.60 &                               (-inf, inf) &        float \\
max\_position\_start     &    -0.40 &                               (-inf, inf) &        float \\
max\_speed              &     0.07 &                                  (0, inf) &        float \\
max\_velocity\_start     &     0.00 &                               (-inf, inf) &        float \\
min\_position           &    -1.20 &                               (-inf, inf) &        float \\
min\_position\_start     &    -0.60 &                               (-inf, inf) &        float \\
min\_velocity\_start     &     0.00 &                               (-inf, inf) &        float \\
goal\_position          &     0.45 &                               (-inf, inf) &        float \\
goal\_velocity          &     0.00 &                               (-inf, inf) &        float \\
max\_position           &     0.60 &                               (-inf, inf) &        float \\
max\_position\_start     &    -0.40 &                               (-inf, inf) &        float \\
max\_speed              &     0.07 &                                  (0, inf) &        float \\
max\_velocity\_start     &     0.00 &                               (-inf, inf) &        float \\
min\_position           &    -1.20 &                               (-inf, inf) &        float \\
min\_position\_start     &    -0.60 &                               (-inf, inf) &        float \\
min\_velocity\_start     &     0.00 &                               (-inf, inf) &        float \\
power                  &     0.00 &                               (-inf, inf) &        float \\
dt                     &     0.05 &                                  (0, inf) &        float \\
g                      &    10.00 &                                  (0, inf) &        float \\
initial\_angle\_max      &     3.14 &                                  (0, inf) &        float \\
initial\_velocity\_max   &     1.00 &                                  (0, inf) &        float \\
l                      &     1.00 &                              (1e-06, inf) &        float \\
m                      &     1.00 &                              (1e-06, inf) &        float \\
max\_speed              &     8.00 &                               (-inf, inf) &        float \\
FPS                    &    50.00 &                                  (1, 500) &        float \\
FRICTION               &     2.50 &                                   (0, 10) &        float \\
GRAVITY\_X              &     0.00 &                                 (-20, 20) &        float \\
GRAVITY\_Y              &   -10.00 &                              (-20, -0.01) &        float \\
INITIAL\_RANDOM         &     5.00 &                                   (0, 50) &        float \\
LEG\_DOWN               &    -0.27 &                               (-2, -0.25) &        float \\
LEG\_H                  &     1.13 &                                 (0.25, 2) &        float \\
LEG\_W                  &     0.27 &                               (0.25, 0.5) &        float \\
LIDAR\_RANGE            &     5.33 &                                 (0.5, 20) &        float \\
MOTORS\_TORQUE          &    80.00 &                                  (0, 200) &        float \\
SCALE                  &    30.00 &                                  (1, 100) &        float \\
SPEED\_HIP              &     4.00 &                               (1e-06, 15) &        float \\
SPEED\_KNEE             &     6.00 &                               (1e-06, 15) &        float \\
TERRAIN\_GRASS          &    10.00 &                                   (5, 15) &          int \\
TERRAIN\_HEIGHT         &     5.00 &                                   (3, 10) &        float \\
TERRAIN\_LENGTH         &   200.00 &                                (100, 500) &          int \\
TERRAIN\_STARTPAD       &    20.00 &                                  (10, 30) &          int \\
TERRAIN\_STEP           &     0.47 &                                 (0.25, 1) &        float \\
VIEWPORT\_H             &   400.00 &                                (200, 800) &          int \\
VIEWPORT\_W             &   600.00 &                               (400, 1000) &          int \\
FPS                    &    50.00 &                                  (1, 500) &        float \\
GRAVITY\_X              &     0.00 &                                 (-20, 20) &        float \\
GRAVITY\_Y              &   -10.00 &                              (-20, -0.01) &        float \\
INITIAL\_RANDOM         &  1000.00 &                                 (0, 2000) &        float \\
LEG\_AWAY               &    20.00 &                                   (0, 50) &        float \\
LEG\_DOWN               &    18.00 &                                   (0, 50) &        float \\
LEG\_H                  &     8.00 &                                   (1, 20) &        float \\
LEG\_SPRING\_TORQUE      &    40.00 &                                  (0, 100) &        float \\
LEG\_W                  &     2.00 &                                   (1, 10) &        float \\
MAIN\_ENGINE\_POWER      &    13.00 &                                   (0, 50) &        float \\
SCALE                  &    30.00 &                                  (1, 100) &        float \\
SIDE\_ENGINE\_AWAY       &    12.00 &                                   (1, 20) &        float \\
SIDE\_ENGINE\_HEIGHT     &    14.00 &                                   (1, 20) &        float \\
SIDE\_ENGINE\_POWER      &     0.60 &                                   (0, 50) &        float \\
VIEWPORT\_H             &   400.00 &                                (200, 800) &          int \\
VIEWPORT\_W             &   600.00 &                               (400, 1000) &          int \\
VEHICLE                &     0.00 &                                         - &  categorical \\
actuator\_strength      &   300.00 &                                  (1, inf) &        float \\
angular\_damping        &    -0.05 &                               (-inf, inf) &        float \\
friction               &     0.60 &                               (-inf, inf) &        float \\
gravity                &    -9.80 &                              (-inf, -0.1) &        float \\
joint\_angular\_damping  &    35.00 &                                  (0, inf) &        float \\
joint\_stiffness        &  5000.00 &                                  (1, inf) &        float \\
torso\_mass             &    10.00 &                                (0.1, inf) &        float \\
actuator\_strength      &   300.00 &                                  (1, inf) &        float \\
angular\_damping        &    -0.05 &                               (-inf, inf) &        float \\
friction               &     0.60 &                               (-inf, inf) &        float \\
gravity                &    -9.80 &                              (-inf, -0.1) &        float \\
joint\_angular\_damping  &    35.00 &                                  (0, inf) &        float \\
joint\_stiffness        &  5000.00 &                                  (1, inf) &        float \\
target\_distance        &    15.00 &                                (0.1, inf) &        float \\
target\_radius          &     2.00 &                                (0.1, inf) &        float \\
torso\_mass             &     1.00 &                                (0.1, inf) &        float \\
actuator\_strength      &   300.00 &                                  (1, inf) &        float \\
angular\_damping        &    -0.05 &                               (-inf, inf) &        float \\
friction               &     0.60 &                               (-inf, inf) &        float \\
gravity                &    -9.80 &                              (-inf, -0.1) &        float \\
joint\_angular\_damping  &    50.00 &                                  (0, inf) &        float \\
joint\_stiffness        &  5000.00 &                                  (1, inf) &        float \\
target\_distance        &    10.00 &                                (0.1, inf) &        float \\
target\_height          &     8.00 &                                (0.1, inf) &        float \\
target\_radius          &     1.10 &                                (0.1, inf) &        float \\
angular\_damping        &    -0.05 &                               (-inf, inf) &        float \\
friction               &     0.60 &                               (-inf, inf) &        float \\
gravity                &    -9.80 &                              (-inf, -0.1) &        float \\
joint\_angular\_damping  &    20.00 &                                  (0, inf) &        float \\
joint\_stiffness        & 15000.00 &                                  (1, inf) &        float \\
torso\_mass             &     9.46 &                                (0.1, inf) &        float \\
angular\_damping        &    -0.05 &                               (-inf, inf) &        float \\
friction               &     0.60 &                               (-inf, inf) &        float \\
gravity                &    -9.80 &                              (-inf, -0.1) &        float \\
joint\_angular\_damping  &    20.00 &                                  (0, inf) &        float \\
torso\_mass             &     8.91 &                                (0.1, inf) &        float \\
actuator\_strength      &   100.00 &                                  (1, inf) &        float \\
angular\_damping        &    -0.05 &                               (-inf, inf) &        float \\
friction               &     0.60 &                               (-inf, inf) &        float \\
gravity                &    -9.81 &                              (-inf, -0.1) &        float \\
joint\_angular\_damping  &    50.00 &                                  (0, 360) &        float \\
joint\_stiffness        & 40000.00 &                                  (1, inf) &        float \\
target\_distance        &     0.50 &                               (0.01, inf) &        float \\
target\_radius          &     0.02 &                               (0.01, inf) &        float \\
torso\_mass             &     1.00 &                                  (0, inf) &        float \\
actuator\_strength      &     1.00 &                                  (0, inf) &        float \\
density                &  5000.00 &                                  (0, inf) &        float \\
friction\_rolling       &     1.00 &                                  (0, inf) &        float \\
friction\_tangential    &     1.00 &                                  (0, inf) &        float \\
friction\_torsional     &     1.00 &                                  (0, inf) &        float \\
geom\_density           &     1.00 &                                  (0, inf) &        float \\
gravity                &    -9.81 &                              (-inf, -0.1) &        float \\
joint\_damping          &     1.00 &                                  (0, inf) &        float \\
joint\_stiffness        &     0.00 &                                  (0, inf) &        float \\
limb\_length\_0          &     0.17 &                               (0.01, 0.2) &        float \\
limb\_length\_1          &     0.16 &                               (0.01, 0.2) &        float \\
spinner\_length         &     0.18 &                               (0.01, 0.4) &        float \\
spinner\_radius         &     0.04 &                              (0.01, 0.05) &        float \\
timestep               &     0.00 &                              (0.001, 0.1) &        float \\
viscosity              &     0.00 &                                  (0, inf) &        float \\
wind\_x                 &     0.00 &                               (-inf, inf) &        float \\
wind\_y                 &     0.00 &                               (-inf, inf) &        float \\
wind\_z                 &     0.00 &                               (-inf, inf) &        float \\
actuator\_strength      &     1.00 &                                  (0, inf) &        float \\
density                &  5000.00 &                                  (0, inf) &        float \\
friction\_rolling       &     1.00 &                                  (0, inf) &        float \\
friction\_tangential    &     1.00 &                                  (0, inf) &        float \\
friction\_torsional     &     1.00 &                                  (0, inf) &        float \\
geom\_density           &     1.00 &                                  (0, inf) &        float \\
gravity                &    -9.81 &                              (-inf, -0.1) &        float \\
joint\_damping          &     1.00 &                                  (0, inf) &        float \\
joint\_stiffness        &     0.00 &                                  (0, inf) &        float \\
timestep               &     0.00 &                              (0.001, 0.1) &        float \\
viscosity              &     0.00 &                                  (0, inf) &        float \\
wind\_x                 &     0.00 &                               (-inf, inf) &        float \\
wind\_y                 &     0.00 &                               (-inf, inf) &        float \\
wind\_z                 &     0.00 &                               (-inf, inf) &        float \\
actuator\_strength      &     1.00 &                                  (0, inf) &        float \\
density                &     0.00 &                                  (0, inf) &        float \\
friction\_rolling       &     1.00 &                                  (0, inf) &        float \\
friction\_tangential    &     1.00 &                                  (0, inf) &        float \\
friction\_torsional     &     1.00 &                                  (0, inf) &        float \\
geom\_density           &     1.00 &                                  (0, inf) &        float \\
gravity                &    -9.81 &                              (-inf, -0.1) &        float \\
joint\_damping          &     1.00 &                                  (0, inf) &        float \\
joint\_stiffness        &     0.00 &                                  (0, inf) &        float \\
timestep               &     0.01 &                              (0.001, 0.1) &        float \\
viscosity              &     0.00 &                                  (0, inf) &        float \\
wind\_x                 &     0.00 &                               (-inf, inf) &        float \\
wind\_y                 &     0.00 &                               (-inf, inf) &        float \\
wind\_z                 &     0.00 &                               (-inf, inf) &        float \\
actuator\_strength      &     1.00 &                                  (0, inf) &        float \\
density                &     0.00 &                                  (0, inf) &        float \\
friction\_rolling       &     1.00 &                                  (0, inf) &        float \\
friction\_tangential    &     1.00 &                                  (0, inf) &        float \\
friction\_torsional     &     1.00 &                                  (0, inf) &        float \\
geom\_density           &     1.00 &                                  (0, inf) &        float \\
gravity                &    -9.81 &                              (-inf, -0.1) &        float \\
joint\_damping          &     1.00 &                                  (0, inf) &        float \\
joint\_stiffness        &     0.00 &                                  (0, inf) &        float \\
timestep               &     0.00 &                              (0.001, 0.1) &        float \\
viscosity              &     0.00 &                                  (0, inf) &        float \\
wind\_x                 &     0.00 &                               (-inf, inf) &        float \\
wind\_y                 &     0.00 &                               (-inf, inf) &        float \\
wind\_z                 &     0.00 &                               (-inf, inf) &        float \\
\bottomrule
\end{tabular}
\end{table}


==> tables/context_features/context_features_defaults_bounds_CARLMountainCarContinuousEnv.tex <==
\begin{subtable}{0.4\textwidth}
\centering
\caption[CARLMountainCarContinuousEnv]{CARLMountainCarContinuousEnv}
\label{tab:context_features_defaults_bounds_CARLMountainCarContinuousEnv}
\begin{tabular}{lrll}
\toprule
   Context Feature &  Default &      Bounds &  Type \\
\midrule
     goal\_position &     0.45 & (-inf, inf) & float \\
     goal\_velocity &     0.00 & (-inf, inf) & float \\
      max\_position &     0.60 & (-inf, inf) & float \\
max\_position\_start &    -0.40 & (-inf, inf) & float \\
         max\_speed &     0.07 &    (0, inf) & float \\
max\_velocity\_start &     0.00 & (-inf, inf) & float \\
      min\_position &    -1.20 & (-inf, inf) & float \\
min\_position\_start &    -0.60 & (-inf, inf) & float \\
min\_velocity\_start &     0.00 & (-inf, inf) & float \\
             power &     0.00 & (-inf, inf) & float \\
\bottomrule
\end{tabular}
\end{subtable}


==> tables/overview_benchmarks.tex <==
\newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
\begin{table}[]
    \small{
    \centering
    \caption{Benchmark collections in Meta-RL}
    \label{tab:overview_benchmarks_related_work}
    \begin{tabular}{P{2cm}P{2.3cm}P{2.5cm}P{2.3cm}P{2cm}}
    \toprule
        Benchmark &  Goal & Environments & Variations of the Task & Access \\
        \midrule
        \addlinespacetable
        MDP Playground~\citep{rajan-arxiv19} 
        & AutoRL \& Characterization of RL algorithms 
        & Toy settings \& MuJoCo/Atari extensions
        & Properties of RL problems (e.g. reward delay) 
        & open-source (except for MuJoCo wrapper)  \\
        %\hline
        bsuite ~\citep{osband-iclr20} 
        & Characterization of RL algorithms 
        & Bandits \& Classic Control
        & Fixed experiments
        & open-source
        \\
        %\hline
        \addlinespacetable
        ALE \citep{machado-jair28} 
        & Transfer within ALE tasks
        & Arcade game environments
        & Fixed experiments (flavors)
        & open-source \\
        %\hline
        \addlinespacetable
        ProcGen \citep{cobbe-2019} 
        & Generalization
        & Arcade Games 
        & Procedurally generated levels
        & open-source \\
        %\hline
        \addlinespacetable
        Alchemy \citep{wang-corr21} 
        & Generalization \& skill acquisition
        & Standard and simplified alchemy environment
        & Distribution across levels
        & open-source\\
        %\hline
        \addlinespacetable
        Meta-world \citep{yu-corl19} 
        & Transfer Learning 
        & Hand Manipulation tasks
        & Standardized sets of tasks
        & closed-source (MuJoCo required)\\
        %\hline
        \addlinespacetable
        MTEnv \citep{sodhani-2021} 
        & Transfer Learning, Representation Learning \& Generalization
        & Toy Settings, Meta-world, Block MDP enironments
        & Fixed settings
        & closed-source (MuJoCo required)\\
        %\hline
        \addlinespacetable
        Safety Gym \citep{ray-2019} 
        & Safe RL
        & Robot navigation with hazards
        & Several configurable features per task
        & closed-source (MuJoCo required)\\
        %\hline
        \addlinespacetable
        TeachMyAgent \citep{romac-icml21} 
        & Student-Teacher Curriculum Learning
        & Box2D tasks with several different walkers each
        & Task distribution with increasing difficulty
        & open-source\\
        %\hline
        \addlinespacetable
        Offworld Gym \citep{offworldgym} 
        & Training on a real robot
        & Robot navigation
        & Discrete \& continuous
        & open-source \\
        %\hline
        \midrule
        \addlinespacetable
        \GenRL (ours)
        & Generalization
        & Classic Control, Box2D, Brax robots, game playing, RNA design
        & Several configurable features per task
        & open-source \\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/rel_work_tab.tex <==
% \newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
% \newcommand{\addlinespacetable}[0]{\addlinespace[0.01cm]}
% \begin{table}[]
%     \small{
%     \centering
%     \caption{Comparison of the \GenRL Benchmark collection to related Benchmarks}
%     \label{tab:comparison_benchmarks_related_work}
%     \begin{tabular}{l cc cc cc}
%     \toprule
%         Benchmark &  Open Source & Explicit Context & Cheap Training & Diverse Tasks & Varying $\mathcal{T}$ & Varying $\mathcal{R}$ \\
%         \midrule
%         \addlinespacetable
%         MDPP~\citep{rajan-arxiv19} 
%         & \ok
%         & \ok
%         & \tick
%         & \tick
%         & \tick
%         & \tick
%         \\
%         %\hline
%         bsuite ~\citep{osband-iclr20} 
%         & \tick
%         & \cross
%         & \tick
%         & \tick
%         & \cross
%         & \cross
%         \\
%         %\hline
%         \addlinespacetable
%         ALE \citep{machado-jair28} 
%         & \tick
%         & \cross
%         & \ok
%         & \ok
%         & \cross
%         & \cross
%         \\
%         %\hline
%         \addlinespacetable
%         ProcGen \citep{cobbe-2019} 
%         & \tick
%         & \cross
%         & \cross
%         & \tick
%         & \tick
%         & \cross
%         \\
%         %\hline
%         \addlinespacetable
%         Alchemy \citep{wang-corr21} 
%         & \tick
%         & \ok
%         & \cross
%         & \ok
%         & \tick
%         & \tick
%         \\
%         %\hline
%         \addlinespacetable
%         Meta-world \citep{yu-corl19} 
%         & \cross
%         & \tick
%         & \cross
%         & \ok
%         & \ok
%         & \tick
%         \\
%         %\hline
%         \addlinespacetable
%         MTEnv \citep{sodhani-2021} 
%         & \cross
%         & \tick
%         & \cross
%         & \ok
%         & \ok
%         & \tick
%         \\
%         %\hline
%         \addlinespacetable
%         Safety Gym \citep{ray-2019} 
%         & \cross
%         & \cross
%         & \cross
%         & \ok
%         & \tick
%         & \tick
%         \\
%         %\hline
%         \addlinespacetable
%         TeachMyAgent \citep{romac-icml21} 
%         & \tick
%         & \ok
%         & \cross
%         & \ok
%         & \tick
%         & \tick
%         \\
%         %\hline
%         % \addlinespacetable
%         % Offworld Gym \citep{offworldgym} 
%         % & \tick
%         % & \cross
%         % & \cross
%         % & \cross
%         % & \cross
%         % & \cross
%         % \\
%         %\hline
%         \midrule
%         \addlinespacetable
%         \GenRL (ours)
%         & \tick
%         & \tick
%         & \tick
%         & \tick
%         & \tick
%         & \tick
%         \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{table}


\newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcommand{\addlinespacetable}[0]{\addlinespace[0.01cm]}
\begin{table}[tbp]
    \small{
    \centering
    \caption{Comparison of the \GenRL Benchmark collection to related Benchmarks. Benchmarks are rated as true (\tick), somewhat true (\ok) or false (\cross) in each category.}
    \label{tab:comparison_benchmarks_related_work}
    \begin{tabular}{l cc cc c}
    \toprule
        Benchmark &  Open Source & Explicit Context & Cheap Training\footnotemark & Diverse Tasks & Varying $\mathcal{T} \& \mathcal{R}$ \\
        \midrule
        \addlinespacetable
        MDPP~\citep{rajan-arxiv19} 
        & \ok
        & \ok
        & \tick
        & \tick
        & \tick
        \\
        %\hline
        bsuite ~\citep{osband-iclr20} 
        & \tick
        & \cross
        & \tick
        & \tick
        & \cross
        \\
        %\hline
        \addlinespacetable
        ALE \citep{machado-jair28} 
        & \tick
        & \cross
        & \ok
        & \ok
        & \cross
        \\
        %\hline
        \addlinespacetable
        ProcGen \citep{cobbe-2019} 
        & \tick
        & \cross
        & \cross
        & \tick
        & \cross
        \\
        %\hline
        \addlinespacetable
        Alchemy \citep{wang-corr21} 
        & \tick
        & \ok
        & \cross
        & \ok
        & \tick
        \\
        %\hline
        \addlinespacetable
        Meta-world \citep{yu-corl19} 
        & \cross
        & \tick
        & \cross
        & \ok
        & \ok
        \\
        %\hline
        \addlinespacetable
        MTEnv \citep{sodhani-2021} 
        & \cross
        & \tick
        & \cross
        & \ok
        & \ok
        \\
        %\hline
        \addlinespacetable
        Safety Gym \citep{ray-2019} 
        & \cross
        & \cross
        & \cross
        & \ok
        & \tick
        \\
        %\hline
        \addlinespacetable
        TMA \citep{romac-icml21} 
        & \tick
        & \ok
        & \cross
        & \ok
        & \tick
        \\
        \addlinespacetable
        MiniGrid \citep{gym_minigrid}
        & \tick
        & \cross
        & \tick
        & \tick
        & \ok
        \\
        \addlinespacetable
        NetHack \citep{kuttler-neurips20}
        & \tick
        & \ok
        & \cross
        & \tick
        & \cross
        \\
        \addlinespacetable
        MiniHack \citep{samvelyan2021minihack}
        & \tick
        & \ok
        & \tick
        & \tick
        & \tick
        \\
        %\hline
        % \addlinespacetable
        % Offworld Gym \citep{offworldgym} 
        % & \tick
        % & \cross
        % & \cross
        % & \cross
        % & \cross
        % & \cross
        % \\
        %\hline
        \midrule
        \addlinespacetable
        \GenRL (ours)
        & \tick
        & \tick
        & \tick
        & \tick
        & \tick
        \\
    \bottomrule
    \end{tabular}
    }
\end{table}
